MS*: A New Exact Algorithm for Multi-agent Simultaneous Multi-goal Sequencing and Path Finding

In multi-agent applications such as surveillance and logistics, fleets of mobile agents are often expected to coordinate and safely visit a large number of goal locations as efficiently as possible. The multi-agent planning problem in these applications involves allocating and sequencing goals for each agent while simultaneously producing conflict-free paths for the agents. In this article, we introduce a new algorithm called MS* which computes an optimal solution for this multi-agent problem by fusing and advancing state of the art solvers for multi-agent path finding (MAPF) and multiple travelling salesman problem (mTSP). MS* leverages our prior subdimensional expansion approach for MAPF and embeds the mTSP solvers to optimally allocate and sequence goals for agents. Numerical results show that our new algorithm can solve the multi-agent problem with 20 agents and 50 goals in a minute of CPU time on a standard laptop.

==> analysis-old.tex <==

As discussed in the remark above, we will provide a short proof of the theoretical properties of MS*-c assuming the (multi-)goal sequencing procedure returns an optimal solution. 

\vspace{0.1cm}

\begin{lemma}\label{lem:transform}
	Given a search state $s$ and $G$, let $cost(\tau_*)$ denote the cost of the tour $\tau_*$ computed by the goal sequencing procedure in the transformed graph $G'$ and let $\pi_m(v(s),v_f)$ denote a joint path in $G$ with the minimum cost that starts from$s$, visits all un-visited goals and ends at destinations. Then $cost(\tau_*) = g(\pi_m(v(s),v_f))$.
\end{lemma}

\begin{proof}
It is known from \cite{oberlin2009transformation} that the optimal cost of finding $N$ goal sequences for the agents spanning the nodes in $G'$ is equal to the cost of the shortest TSP tour in $G'$. The Lemma follows.

\begin{comment}
	First of all, given a minimal cost joint path $\pi_{m}(v,v_g)$ starting at state $s=(v,a)$ that visits all un-visited targets and end at goals, we show that the cost of this joint path $g(\pi_{m}(v,v_g))$ is no less than $cost(\tau_*)$. With such a path $\pi_{m}(v,v_g)$, by adding $N$ zero-cost edges to connect $v^i_g$ with $v^{i+1}_o, i \in\{1,2,\dots, N-1\}$ and $v^N_g$ with $v^{1}_o$, we get a corresponding tour $\tau_{m}$ in transformed graph $G'$ and the cost of this constructed tour $cost(\tau_m)$ in $G'$ is the same as $g(\pi_m(v,v_g))$. Since $\tau_{m}$ is not guaranteed to be optimal in $G'$, $cost(\tau_m)$ must be no less than the cost of the optimal tour in $G'$, $i.e.$ $cost(\tau_m) \geq cost(\tau_*)$. Therefore,
	\begin{eqnarray}\label{lem:transform:eqn1}
		g(\pi_m(v,v_g)) = cost(\tau_m) \geq cost(\tau_*).
	\end{eqnarray}
	
	Secondly, given the optimal tour $\tau_*$ in $G'$, as described in Section \ref{sec:task_seq} and \ref{sec:heu_and_policy}, there is a corresponding induced joint path $\pi_\gamma(v,v_g)$ with cost $g(\pi_\gamma(v,v_g)) = cost(\tau_*)$. Because $\pi_\gamma(v,v_g)$ is not guaranteed to be a minimal cost path $\pi_{m}(v,v_g)$ in $G$, we have $g(\pi_\gamma(v,v_g)) \geq g(\pi_m(v,v_g))$ and therefore,
	\begin{eqnarray}\label{lem:transform:eqn2}
		cost(\tau_*) = g(\pi_\gamma(v,v_g)) \geq g(\pi_m(v,v_g)).
	\end{eqnarray}
	Put (\ref{lem:transform:eqn1}) and (\ref{lem:transform:eqn2}) together, we have $cost(\tau_*) = g(\pi_m(v,v_g))$.
	\end{comment}
\end{proof}

\vspace{0.1cm}

\begin{lemma}\label{lem:no_sol}
    If there is no feasible solution, MS*-c reports failure in finite time.
\end{lemma}
\begin{proof}
    There is a finite number of states and at each state $s$, the collision set $I_C(s)$ can be modified at most once ($I_C(s)$ is either $\emptyset$ or $I_N$). Thus the sub-space searched by MS*-c will be at most modified for a finite time. Within this sub-space, MS*-c conducts heuristic search (A*-like search) with state dominance pruning. Therefore, if there is no solution, MS*-c terminates in finite time.
\end{proof}

\vspace{0.1cm}

\begin{theorem}\label{thm:optimal}
    MS*-c either computes the optimal solution for MSMP or report failure in finite time.
\end{theorem}
\begin{proof}
    With Lemma \ref{lem:transform}, if there is no conflict, MS* restricts the agents to travel along the joint path computed by the goal sequencing procedure and the resulting solution is guaranteed to be optimal. If there are conflicts at state $s$ along the solution, with Algorithm \ref{alg.backprop}, all ancestor states of $s$ are updated with $I_C=I_N$ and re-inserted into OPEN for re-expansion with all possible moves considered. Among all those moves, MS*-c uses an underestimating heuristic to prioritizes and expands states (just like A*) and is therefore guaranteed to be optimal.
    With Lemma \ref{lem:no_sol}, if there is no solution, MS*-c reports failure in finite time.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% BELOW are all comments !!!!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

M* terminates in finite time if the configuration space is finite and the collision set can be grown for a finite number of times, which makes the algorithm terminates in finite time if there is no solution.
In MS*, since $G$ is a finite graph, the state space that consists of all possible combination of joint vertices and assignment vectors is also finite and the collision set defined at each state can grow for a finite number of times, thus MS* terminates in finite time if there is not solution.

In M*, A* search is used to find individual optimal path for each agent $i$ connecting its pre-defined start and goal ignoring any other agents. The computed optimal path provides heuristic for agent $i$ as well as the optimal policy for agent $i$ to follow if there is not conflict. M* begins by letting agents follow their optimal policies and only consider all possible neighbors for an agent if the agent is involved collision.
In addition, M* select candidate state in OPEN in an order based on the $f$-value of states. As long as the heuristic of any state is an underestimate, M* is guaranteed to find the optimal solution, if exists. 
Therefore, in MS*, if it can be shown that task sequencing satisfies the following two requirements:
\begin{itemize}
	\item (R1) optimal policies that leads to optimal path if no agent-agent collision happens,
	\item (R2) heuristics that underestimates the cost-to-go for all states,
\end{itemize}
MS* is then guaranteed to be complete and optimal. 

To support requirement (1), let's introduce the following lemma which describes the property of the transformation we introduced. 
\begin{lemma}\label{lem:transform}
	Given a search state $s_k = (v_k, a_k)$ and $G^w$, let $cost(\tau_*)$ denote the cost of the optimal tour $\tau_*$ in transformed graph $G'$ and let $C_\pi$ denote the sum of cost over all paths $\pi^i_*(v^i_l,v^i_{l+1}), l = 1,2,\dots, \ell^i, \forall i \in I_N$ induced by $\gamma^i, i \in I_N$, then $cost(\tau_*) = C_\pi$.
\end{lemma}

Detailed proof of Lemma \ref{lem:transform} can be found in our prior work \cite{oberlin2009transformation}. To make the article self-contained, a sketch proof is provided here. {\color{red}Not sure if we need a sketch proof or just let the reader to find in reference. We are already running out of space...}

\begin{proof}
	First of all, given an arbitrary sequence of path $\pi^i_*(v^i_l,v^i_{l+1}), l = 1,2,\dots, \ell^i, \forall i \in I_N$ that visits all targets and end at goals, we show that the cost of all paths $C_\pi$ is no less than $cost(\tau_*)$. For every agent $i \in I_N$, connecting paths $\pi^i_*(v^i_l,v^i_{l+1}), l = 1,2,\dots, \ell^i$ leads to $N$ paths $\pi^i(v_k,v_g)$ that visits all targets and end up at a goal. By adding $N$ zero-cost edges to connect $v^i_g$ with $v^{i+1}_o, i \in\{1,2,\dots, N-1\}$ and $v^N_g$ with $v^{1}_o$, we get a tour $\tau$ in transformed graph $G'$ and the cost of this constructed tour $cost(\tau)$ is the same as $C_\pi$. In addition, $cost(\tau)$ must be no larger than the optimal tour in $G'$, $i.e.$ $cost(\tau) \geq cost(\tau_*)$. Therefore,
	\begin{eqnarray}\label{lem:transform:eqn1}
		C_\pi \geq cost(\tau_*).
	\end{eqnarray}
	Secondly, given the optimal tour $\tau_*$ in $G'$, by the construction of a transformed graph $G'$, all edges $(v'_a,v'_b), v'_a \in V^w_g, v'_b \in v_k$ are zero-cost while edges $(v'_a,v'_b), v'_a \in V'\backslash V^w_g, v'_b \in v_k$ have infinite cost. Therefore, there are $N$ zero-cost edges $(v'_{a^i},v'_{b^i}), i \in I_N$ in $\tau_*$ with $v'_{a^i} \in V^w_g$ and $v'_{b^i} \in v_k$ because otherwise $\tau_*$ cannot be optimal. Removing all those zero-cost edges divides $\tau_*$ into $N$ path segments in $G'$, each of which has a cost no less than the cost of the optimal path in $G^w$. Therefore, $cost(\tau_*)$ is no less than the sum of optimal individual paths for agents in $G^w$. Therefore,
	\begin{eqnarray}\label{lem:transform:eqn2}
		cost(\tau_*) \geq C_\pi.
	\end{eqnarray}
	Put (\ref{lem:transform:eqn1}) and (\ref{lem:transform:eqn2}) together, we have $cost(\tau_*) = C_\pi$.
\end{proof}

With Lemma \ref{lem:transform}, requirement R1 follows immediately. Since the heuristic is induced from task sequencing ignoring potential agent-agent conflicts, requirement R2 is also satisfied. Therefore, we conclude this section with the following theorem.

\begin{theorem}\label{thm:optimal}
	MS* is complete and optimal for MSTP problem.
\end{theorem}

\end{comment}

==> result-old.tex <==

\subsection{Simulation Settings}\label{sec:experiment_settings}

To numerically evalute MS*-c and MS*, we implemented the algorithms in Python and tested them on a computer with a CPU of 2.5 GHz Intel Core i7 and 16GB RAM. We generated five different 32x32 four-connected grids with 20\% random obstacles. %, as shown in Figure \ref{fig:grids}. 
For each grid, 20 test cases were generated with random starts and goals for a set of $N$ agents with $N=5,10,20$ and a set of $M$ targets with $M=10,20,30,40,50$.
In total, there are 100 test cases over five different grids for each number of agents $N$.
For each test instance, we limit the search time of the algorithms to {\bf one minute} and measure the success rates of the algorithms within this time bound. 

We tested MS* and MS*-c, and they return the same solution cost for any instance when both of them succeed. In addition, the success rate of MS* is higher than MS*-c for less than 5\% for all the tested instances. Therefore, we report only the results related to MS* in the following text.

%\begin{figure}
%	\centering
%	\vspace{-3mm}
%	\includegraphics[width=.5\linewidth]{grids_0p2_0.png}
%	\hspace{-6mm}
%	\includegraphics[width=.5\linewidth]{grids_0p2_1.png}
%	\hspace{-6mm}
%	\includegraphics[width=.5\linewidth]{grids_0p2_2.png}
%	\hspace{-6mm}
%	\includegraphics[width=.5\linewidth]{grids_0p2_3.png}
%	\hspace{-6mm}
%	\includegraphics[width=.5\linewidth]{grids_0p2_4.png}
%	\hspace{-3mm}
%	\vspace{-3mm}
%	\caption{Test grids with 20\% random obstacles.}
%	\label{fig:grids}
%\end{figure}

% \begin{figure}
% 	\centering
% 	\hspace{-10mm}
% 	\vspace{-1mm}
% 	\includegraphics[width=\linewidth]{test_case_eg.png}
% 	\vspace{-3mm}
% 	\hspace{-10mm}
% 	\caption{An example of test instances with 20 agents and 50 targets where starts of agents are marked with green circles, targets are marked with blue triangles and goals are marked with red stars.}
% 	\label{fig:test_case}
% \end{figure}

\subsection{Success Rate}\label{sec:succ_rate}
As shown in Figure \ref{fig:succ_rate}, as $M$ increases, with $N=5,10$ agents, MS* achieves success rates greater than 80\% and stays relatively stable. For more number of agents ($N=20$), the success rate significantly decreases as the number of targets reaches 50. For most test instances with a smaller number of agents, task sequencing provides policies move agents along paths that are conflict-free. When there are more agents (e.g. $N=20$), the chances that agents collide following the task sequencing policies increase which results in more computation and lowers the success rate.

\begin{figure}
	\centering
	\hspace{-10mm}
	\vspace{-1mm}
	\includegraphics[width=0.9\linewidth]{mtspf_32x32_obst0p2_success_rate_xM.png}
	\vspace{-3mm}
	\hspace{-10mm}
	\caption{Success rates of MS* as a function of the number of agents ($N$) and number of targets ($M$) within one minute computation time. }
	\label{fig:succ_rate}
\end{figure}

\subsection{Task Sequencing Time}\label{sec:tsp_time}
To get a better sense of the computational burden of task sequencing in MS*, we measured the computation time of each task sequencing call and took the average over all the succeeded test instances. From Figure \ref{fig:avg_tsp_time}, as one can expect, as $N$ or $M$ increases, each call of task sequencing takes more time. When $M=50$ and $N=20$, there are $20\text{ agents}+50\text{ targets}+20\text{ goals}=90$ vertices in the transformed graph $G'$ and each task sequencing call requires approximately 30 seconds which is more than half of the time limit. It means that, for test instances with $M=50$ and $N=20$, MS* can call task sequencing for at most once on average because a second task sequencing call makes the program time out.

\begin{figure}
	\centering
	\hspace{-10mm}
	\vspace{-1mm}
	\includegraphics[width=0.9\linewidth]{mtspf_32x32_obst0p2_tsp_avg_time_xM.png}
	\vspace{-3mm}
	\hspace{-10mm}
	\caption{The computation times required for task sequencing in secs as a function of the number of targets (M). }
	\label{fig:avg_tsp_time}
\end{figure}

\begin{comment}
In addition, we also measure the proportion of computation times spent on task sequencing versus the total computation time. From Figure \ref{fig:tsp_percent}, we observe that as $M$ increases, the task sequencing proportion decreases in general. %However, we want to point out an underlying survivor bias in the tests: only ``simiple'' test instances which requires fewer calls of task sequencing are successfully solve by MS*, and therefore counted. For test instances that require several task sequencing computations, MS* times out and the result is not accounted for.

\begin{figure}
	\centering
	\hspace{-10mm}
	\vspace{-1mm}
	\includegraphics[width=0.9\linewidth]{mtspf_32x32_obst0p2_tsp_percentage_xM.png}
	\vspace{-3mm}
	\hspace{-10mm}
	\caption{Average fractions of the total time spent on task sequencing as a function of the number of targets (M). }
	\label{fig:tsp_percent}
\end{figure}
\end{comment}
